Frequency Selective Augmentation for Video Representation Learning

Recent self-supervised video representation learning methods focus on maximizing the similarity between multiple augmented views from the same video and largely rely on the quality of generated views. However, most existing methods lack a mechanism to prevent representation learning from bias towards static information in the video. In this paper, we propose frequency augmentation (FreqAug), a spatio-temporal data augmentation method in the frequency domain for video representation learning. FreqAug stochastically removes specific frequency components from the video so that learned representation captures essential features more from the remaining information for various downstream tasks. Specifically, FreqAug pushes the model to focus more on dynamic features rather than static features in the video via dropping spatial or temporal low-frequency components. To verify the generality of the proposed method, we experiment with FreqAug on multiple self-supervised learning frameworks along with standard augmentations. Transferring the improved representation to five video action recognition and two temporal action localization downstream tasks shows consistent improvements over baselines.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/table_mk200.tex <==
\begin{table}[!t]
\tabcolsep=0.05cm
%\small
%\tiny
\begin{center}
\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{c|l|c|c|c|c|c}
            \hline
            \multirow{2}{*}{\makecell{Method }} & \multirow{2}{*}{\makecell{Augmentation }} &  \multicolumn{3}{c|}{Finetune} &\multicolumn{2}{c}{Low-shot (10\%)}\\
            \cline{3-7}
            & &  UCF101 & HMDB51 & Diving48 & Gym99 & SSv2 \\
            \hline
            \multirow{3}{*}{\makecell{MoCo}} & Baseline & 87.0 & 56.5 & 67.8 & 29.9 & 25.3\\
            %\cline{2-7}
             & + FreqAug-ST &  \textbf{90.0} & \textbf{61.6} & \textbf{71.0} & 34.8 & \textbf{28.1} \\
            %\cline{2-7}
             & + FreqAug-T &  89.8 & 60.8 & 70.3 & \textbf{35.2} & \textbf{28.1} \\
            \hline
             \multirow{3}{*}{\makecell{BYOL}} & Baseline & 88.4 & 59.8 & 70.3 & 38.7 & 29.5 \\
            %\cline{2-7}
             & + FreqAug-ST & \textbf{90.5} & \textbf{63.2} & 72.4 & 40.7 & 31.2  \\
             %\cline{2-7}
             & + FreqAug-T & \textbf{90.5} & 62.7 & \textbf{72.5} & \textbf{40.8} & \textbf{31.6}  \\

            \hline
        \end{tabular}}
\end{center}
\caption{\textbf{Evaluation results of SlowOnly-50 model pretrained on Mini-Kinetics.} We demonstrate FreqAug with MoCo, and BYOL. Low-shot denotes finetuning with only 10\% of total training samples. Refer to Appendix for SimSiam, SimCLR, and SwAV results}
\label{table:mk200}
\end{table}




==> trash/table_code.tex <==
\begin{algorithm*}[!t]
\begin{minted}[fontsize=\footnotesize]{text}
# x: video, B x C x T x H x W
# p: filter probability
# co_s, co_t: spatial and temporal cutoff freq.
# type_s, type_t: HPF if True else LPF
# fftfreq: calculate FFT sample frequencies
# outer: outer product

def freqaug(x, p, co_s, co_t, type_s, type_t):
    if random() < p: # U(0,1)
        # pass bands
        pass_t = torch.abs(torch.fft.fftfreq(T)) < co_t 
        pass_h = torch.abs(torch.fft.fftfreq(H)) < co_s
        pass_w = torch.abs(torch.fft.fftfreq(W)) < co_s
        
        pass_hw = torch.outer(pass_h, pass_w)
        if type_s:
            pass_hw = torch.logical_not(pass_hw)
            
        if type_t:
            pass_t = torch.logical_not(pass_t)
        
        F = torch.outer(pass_t, pass_hw.view(-1)).view(T, H, W) # filter
        X = torch.fft.fft(x) # FFT, X: spectrum
        X_hat = F * X # filtering
        return torch.fft.ifft(X_hat) # inverse FFT
    else:
        return x
\end{minted}
\caption{FreqAug: Pytorch-like Pseudocode}
\label{alg:code}
\end{algorithm*}

\begin{algorithm*}[!t]
\begin{minted}[fontsize=\footnotesize]{text}
# x: video, B x C x T x H x W
# M: mask parameter
# fftfreq: calculate FFT sample frequencies
# outer: outer product

def random_masking(x, M):
    ft = 1.0 / T
    freq_t = [float(i) * ft for i in range(0, T // 2 + 1)]
    
    band_s = random.choice(freq_t) # choose start point of reject band
    freq_t_end = [f for f in freq_t if band_s + M*ft > f >= band_s]
    band_e = random.choice(freq_t_end) # choose end point of reject band
    
    pass_h = torch.abs(torch.fft.fftfreq(H)) <= 0.5 # pass all spatial freq.
    pass_w = torch.abs(torch.fft.fftfreq(W)) <= 0.5 # pass all spatial freq.
    pass_t_s = torch.abs(torch.fft.fftfreq(T)) >= band_s
    pass_t_e = torch.abs(torch.fft.fftfreq(T)) < band_e

    pass_hw = torch.outer(pass_h, pass_w)
    pass_t = torch.logical_not(pass_t_s * pass_t_e)

    F = torch.outer(pass_t, pass_hw.view(-1)).view(T, H, W)
    X = torch.fft.fft(x) # FFT, X: spectrum
    X_hat = F * X # filtering
    return torch.fft.ifft(X_hat) # inverse FFT

\end{minted}
\caption{Temporal Random Masking: Pytorch-like Pseudocode}
\label{alg:code_rand}
\end{algorithm*}

==> trash/table_cutoff.tex <==
\begin{table}[!t]
\tabcolsep=0.07cm
\begin{center}
\resizebox{\linewidth}{!}{
		\begin{tabular}{c|c|c||c|c|c|c|c}
            \hline
            \multirow{2}{*}{\makecell{Backbone }} & \multirow{2}{*}{\makecell{$T\times \tau$ }} &
             \multirow{2}{*}{\makecell{$f^t_{co}$ }} & \multicolumn{3}{c|}{Finetune} &\multicolumn{2}{c}{Low-shot (10\%)}\\
            \cline{4-8}
            & &  & UCF101 & HMDB51 & Diving48 & Gym99 & SSv2 \\
            \hline
              \multirow{5}{*}{\makecell{SO-18}} & \multirow{5}{*}{\makecell{$16\times 4$}} &
              - & 84.5 & 55.2 & 74.9 & 30.3 & 23.9 \\
             & &  0.05 & 86.5 & 58.8 & 75.0 & 34.2 & 26.4 \\
             & & 0.1 & \textbf{88.7} & 58.8 & \textbf{75.7} & 34.7 & 26.1 \\
             & &  0.15 & 87.6 & \textbf{59.5} & 74.7 & 35.3 & \textbf{26.4} \\
             & &  0.2 & 87.1 & 58.5 & 75.1 & \textbf{36.2} & 26.2 \\
            \hline
            \multirow{5}{*}{\makecell{S3D-G}} & \multirow{5}{*}{\makecell{$32\times 2$}} & 
             - &  89.0 & 59.5 & \textbf{70.1} & 42.1 & 30.5\\
            & &  0.05 & 89.7 & \textbf{63.5} & 69.6 & 42.4 & 31.0 \\
             & &  0.1  & 90.4 & 62.2 & 68.8 & 44.3 & 
             \textbf{31.5} \\
             & &  0.15 & 90.2 & 63.4 & 68.9 & \textbf{45.4} & 30.7 \\
             & &  0.2 & \textbf{90.6} & 62.4 & 68.3 & 45.3 & 30.4 \\
            \hline
        \end{tabular}}
\end{center}
\caption{\textbf{Evaluation results on Mini-Kinetics.} We evaluate FreqAug (FA) with diverse backbones, including SlowOnly-50 (SO-50), SlowOnly-18 (SO-18), R(2+1)D and S3D-G, via finetuning and low-shot learning protocols. Here, $T$: number of frames, $\tau$: input stride. 
}
\label{table:cutoff}
\end{table}

